MORPH: Towards Automated Concept Drift Adaptation for Malware Detection

Concept drift is a significant challenge for malware detection, as the performance of trained machine learning models degrades over time, rendering them impractical. While prior research in malware concept drift adaptation has primarily focused on active learning, which involves selecting representative samples to update the model, self-training has emerged as a promising approach to mitigate concept drift. Self-training involves retraining the model using pseudo labels to adapt to shifting data distributions. In this research, we propose MORPH -- an effective pseudo-label-based concept drift adaptation method specifically designed for neural networks. Through extensive experimental analysis of Android and Windows malware datasets, we demonstrate the efficacy of our approach in mitigating the impact of concept drift. Our method offers the advantage of reducing annotation efforts when combined with active learning. Furthermore, our method significantly improves over existing works in automated concept drift adaptation for malware detection.

==> sections/introduction_old.tex <==
\section{Introduction}
Concept drift refers to the phenomenon where the distribution of the testing dataset deviates from that of the training. In malware detection, concept drift can lead to misclassification and an increase in false positives \cite{garcia2009anomaly,chen2020training}. This phenomenon may arise due to new malware variants, the introduction of novel malicious features, or deliberate attempts by malware authors to evade existing detection methods~\cite{jordaney2017transcend}. 
% Consequently, the features present in the training data may differ significantly from those encountered in testing. 
Over time, the impact of concept drift can deteriorate the effectiveness of machine learning models in security applications, rendering them impractical for prolonged usage \cite{chen2023continuous}. For instance, a malware classification model suffering from concept drift can label benign, harmless critical system files as malicious. Or this model may miss the detection of newly emerging malware variants. Concept drift is not a one-time event, and if not addressed continuously, may progressively impact defenses and create an impression of a false sense of security right before a devastating cyberattack \cite{jordaney2017transcend,andresini2021insomnia}.

Prior research has dealt with the onset of concept drift in various ways~\cite{gama2014survey}. While periodically retraining the models using the latest annotation dataset is an effective way to deal with this problem, it is impractical to obtain enough high-quality annotated datasets for malware detection~\cite{mohaisen2014av,wu2023grim}.
% The most straightforward method is periodically retraining the machine learning model using the latest annotated dataset. However, this approach presents practical challenges, particularly in security-critical applications like malware detection. The first challenge stems from the difficulty of accumulating a sufficient number of high-quality labeled datasets for training the model. Manual annotation of new applications as benign or malicious is a laborious process that requires careful examination of all available features.
% Moreover, adversaries often employ various layers of obfuscation in the code and features, further complicating the annotation task. Consequently, having an ample supply of high-quality annotated datasets ready for model training is often impractical. The second challenge involves determining the frequency of model training. While updating the detection model as frequently as possible is desirable, training complex models such as deep neural networks can be computationally intensive. On the other hand, failing to update the model leaves the system vulnerable to new malware variations.
In the face of limited annotation budgets, active learning has emerged as a widely adopted method for combating concept drift \cite{pendlebury2019tesseract}. Active learning aims to select a subset of representative samples from recent data, considering the challenges of labeling large volumes of data. The fundamental idea behind active learning is choosing samples the model is least confident about or those that deviate significantly from known data distribution~\cite{jordaney2017transcend}. Human experts then annotate these selected samples to ensure high-quality labels. As the model exhibits uncertainty towards these samples, they contribute significantly to adapting the decision boundary rapidly to the shifting data distribution.



% Determining when to retrain the model can be based on detecting a shift in data distribution \cite{yang2021cade} or a degradation in the model's performance \cite{jordaney2017transcend}. A new model is trained when there is a substantial shift in the underlying data distribution or when the current model's performance deteriorates while considering the annotation budget. However, this approach still entails the computational overhead of applying a different model for detecting concept drift at specific intervals. Consequently, many studies in the literature opt to periodically retrain the classifier using active learning at fixed intervals, such as every month. 

% On the other hand, concept drift adaptation methods detect a shift in data distribution or a degradation in the model's performance quality. A new model is trained once there is a sufficient shift in the underlying data distribution or the previous model's performance. Continual learning deals with the problem of catastrophic forgetting, where the model is updated incrementally on new samples while maintaining past knowledge. Since storing all the previous data may not be feasible, a key component in continual learning is storing a subset of the previous dataset for future retraining.



% To address the earlier issues with malware detection, We present MORPH: autoMated cOncept dRift adaPtation algoritHm. Our proposed method can adapt deep neural network models without requiring human annotation beyond the original training dataset. This eliminates the labeling effort requirement. While active learning can reduce the annotation effort, it can still be significant for some use cases. Instead, we use semi-supervised learning to leverage the unlabeled samples, which are more readily available. We use the previously trained model to generate pseudo-labels on new samples. Next, we transfer the knowledge from the previous model to an identical model using knowledge distillation \cite{hinton2015distilling}. We use both the labeled and unlabeled samples for this. As the new model is trained on the latest pseudo-labeled samples, it can adapt to concept drift. Transferring knowledge from the previously trained model makes the model robust against catastrophic forgetting.


% Most prior concept drift detection and adaptation research has been on Android malware. We instead focus on Windows PE malware as this is an under-studied field compared to Android malware. Although there has been a decent amount of work on concept drift adaptation~\cite{yang2021cade,jordaney2017transcend,barbero2022transcending} and active learning for tackling concept drift~\cite{chen2023continuous}, the research on automated concept drift adaptation is scarce. The only prior works on automated concept drift adaptation for malware classification are DroidEvolver \cite{xu2019droidevolver} and its updated DroidEvolver++ \cite{kan2021investigating}. Both of them are designed for Android malware classification. DroidEvolver keeps a pool of five different classification models and uses the prediction of the ensemble as the pseudo-label to identify aging models that diverge from the ensemble prediction. Those models are then retrained to be conformant with the ensemble model.
% Previous studies have primarily focused on selecting divergent samples from the existing data distribution and leveraging them for active learning. For instance, the Transcendent method \cite{jordaney2017transcend} utilized calibrated model uncertainty, estimated through p-value estimation, to identify out-of-distribution (OOD) samples. Another approach, CADE \cite{yang2021cade}, employed contrastive learning to acquire improved representations of benign and malicious samples. By learning embedding representations that group benign samples into one cluster and malicious samples into another, CADE detected OOD samples by comparing their distance from the cluster centroids of the same class. However, new malware families may not be accurately placed alongside other malware samples in the embedding space when they emerge.
% To address this issue, hierarchical contrastive learning was introduced in \cite{chen2023continuous}. This approach aims to learn embedding representations that differentiate malware from benign samples and establish closer proximity between malware samples from the same family compared to those from different families. By achieving a fine-grained separation between samples belonging to distinct malware families, this technique enables new malware families to cluster together more effectively. Consequently, these proposed approaches have the potential to significantly reduce the annotation effort required across various datasets while maintaining a high level of classifier performance.


% In contrast to prior works, we adopt a different strategy. It is usually a lot cheaper to accumulate applications (both benign and malicious) than to annotate them with human experts. For example, the AV-TEST Institute registers over 450,000 new malware and potentially unwanted applications daily.\footnote{\url{https://www.av-test.org/en/statistics/malware/}} While \textcolor{red}{sentence can be clearer, in domains where there is an abundance} there is an abundance of unlabeled samples, which are costly to annotate, semi-supervised learning is one of the most widely used learning paradigms. Semi-supervised learning has been successfully used in many fields of machine learning to leverage large amounts of unlabeled data. However, applying semi-supervised learning has been studied very rarely for malware detection. In this work, we combine semi-supervised learning with active learning to adapt malware detection models to changes in data distribution. While semi-supervised learning can help leverage unlabeled data to improve the performance of a machine-learning model, it is insufficient to address the effect of concept drift. For example, consider applications from an entirely new malware in the test set. When such a new family of malware emerges, there can also be different variants of this malware with minor changes. Suppose the model cannot detect samples of this new malware family (i.e., classifies them as benign). Those samples can not be incorporated with their correct annotation in the semi-supervised learning setting. Furthermore, since those samples would be treated as benign, they will bias the model toward predicting samples from a different malware family as benign in the future. Active learning can identify those samples since samples from a new malware family are expected to differ from those present in the training set, e.g., in the embedding space of a trained neural network. However, annotating malware is a costly endeavor, and usually, only a fraction of those new samples can be annotated. Once the model has been trained on these samples, it can more reliably identify samples from the new malware family. As such, we can use semi-supervised learning to utilize the unlabeled samples and make the predictions more robust against new malware variants.

% Most prior works have been focused on adapting to the onset of concept drift for malware classification. However, this means that models are updated retroactively to account for concept drift that has already taken place. This can make the detection model unreliable until they have been retrained with samples from the new malware family. \textcolor{red}{ What is the connection between the two previous sentences and the adversarial training in the following sentences?} 
% In the context of malware detection, the concept drift is much more likely to happen from a malicious application than a benign one because adversaries are incentivized to avoid detection and incorporate features different from those in the training set. They can also attempt to fool detection methods using adversarial attacks for the same reason. On the other hand, benign applications do not have an incentive to fool detection models to be classified as malicious. Motivated by this observation, we also incorporate adversarial training to make the model robust against future concept drift.

% \textcolor{red}{How will challenge 2 (frequency of training) be addressed? What about the class imbalance issue? It isn't mentioned here. Where is contrastive learning used and why?}

% The contributions of our works are as follows
% \begin{enumerate}
%     \item We propose an algorithm for adapting deep neural networks against concept drift for malware detection.
%     \item Our method works on top of the existing active learning methods for continuous learning for malware detection. While prior works focused on sample selection for active learning, we instead focused on utilizing unlabeled, more readily available samples.
%     \textcolor{red}{What about SSL?}
% \item We investigate using adversarial training to make malware detection models more robust against future concept drifts.
% \end{enumerate}


% Despite efforts to reduce annotation requirements, labeling malware families remains labor-intensive, often demanding hours of effort from security analysts \cite{mohaisen2014av}. Consequently, the advantages gained from selecting a smaller number of samples could be outweighed by the need for malware family label annotation. Moreover, if these labels drift away from the current malware landscape, antivirus engines may incorrectly detect them. To address this challenge, our study adopts a contrastive learning approach that only necessitates binary labels for the malware family. By doing so, we can preserve similar characteristics in the embedding space for the selection of drifted samples. In addition, we introduce several key enhancements to the training process. Firstly, we employ a balanced triplet sampling strategy to mitigate the class imbalance issue inherent in malware datasets. This strategy ensures that each class is adequately represented during training, preventing biases towards the majority class. Secondly, we incorporate the \textit{mixup}~\cite{zhang2017mixup} strategy in conjunction with contrastive learning. Mixup promotes linear behavior and reduces overconfident predictions on unseen samples by interpolating the embeddings. These improvements to the training regime allow us to achieve performance on par with state-of-the-art approaches that require the availability of malware family information, thereby effectively reducing the annotation effort required in our methodology.


% The remaining sections of this paper are organized as follows. Section~\ref{sec:back} provides a comprehensive overview of the background and related work on concept drift, highlighting the challenges and existing approaches in addressing this issue. In Section~\ref{sec:met}, we present our proposed method, detailing the key components and techniques employed to mitigate concept drift in Android malware detection. The dataset utilized in our study is introduced in Section~\ref{sec:data}, outlining its characteristics and relevance to our research. In Section~\ref{sec:exp}, we present the experimental results and discuss the findings, evaluating the performance and effectiveness of our approach. To further analyze the impact of different components in our method, Section~\ref{sec:ablation} presents an ablation study. Finally, Section~\ref{sec:con} concludes the paper, summarizing the contributions, discussing the implications of our findings, and outlining potential avenues for future research.

Most prior concept drift detection and adaptation research has been on Android malware. Although there has been a decent amount of work on concept drift adaptation~\cite{yang2021cade,jordaney2017transcend,barbero2022transcending} and active learning for tackling concept drift~\cite{chen2023continuous}, the research on automated concept drift adaptation is scarce. The only prior works on automated concept drift adaptation for malware classification are DroidEvolver \cite{xu2019droidevolver} and its updated DroidEvolver++ \cite{kan2021investigating}. Both of them are designed for Android malware classification. DroidEvolver keeps a pool of five different classification models and uses the prediction of the ensemble as the pseudo-label to identify aging models that diverge from the ensemble prediction. Those models are then retrained to be conformant with the ensemble model.


In this paper, we address the research gap of automated concept drift adaptation for malware detection. While active learning approaches have been explored for concept drift adaptation in previous works~\cite{yang2021cade,jordaney2017transcend,barbero2022transcending,chen2023continuous}, the research on fully automated concept drift adaptation is limited. Existing works in this domain, such as DroidEvolver~\cite{xu2019droidevolver} and its updated version DroidEvolver++~\cite{kan2021investigating}, focus on Android malware classification using passive-aggressive classifiers. These methods maintain a pool of classification models and utilize ensemble predictions as pseudo-labels to identify aging models that deviate from the ensemble. However, there are fundamental limitations to these automated approaches, as human intervention is required to validate the quality of the model at certain stages. Despite these limitations, automated concept drift adaptation shows promise in reducing the manual labeling effort associated with concept drift. In this study, we investigate the effectiveness of this approach using neural networks, where we leverage pseudo-labels to update the model and subsequently reduce the frequency of active learning updates. Pseudo-labels have been commonly employed in neural networks for semi-supervised learning, effectively utilizing unlabeled data. Although pseudo-labels may introduce some noisy labels, they offer an opportunity for the model to learn from additional datasets and adapt its decision boundaries. By examining the application of automated concept drift adaptation with neural networks, we contribute to the understanding of its effectiveness in the context of malware detection. We take into account the inherent challenges and limitations of this approach, emphasizing the need for human validation of the model's quality. Through this research, we aim to explore the potential of automated concept drift adaptation to alleviate the burden of manual labeling efforts and enhance the adaptability of neural network models to evolving malware patterns.

This paper aims to investigate the effectiveness of combining pseudo-labels with active learning for concept drift adaptation in malware detection. Specifically, We address the following key research questions:

\begin{enumerate}
\item RQ1) \textit{Does pseudo-labeling provide sufficient information for automatic concept drift adaptation in neural network-based malware detection?}

We examine whether pseudo-labeling alone can facilitate automatic adaptation to concept drift in the context of neural network-based malware detection. By leveraging pseudo-labels, which are generated by the model's own predictions, we assess their effectiveness in capturing and adapting to evolving malware patterns without relying solely on manually annotated ground truth labels.

% \item RQ2) \textit{Does contrastive learning improve the selection of pseudo-labels for concept drift adaptation?}

% We explore the impact of contrastive learning on the selection of pseudo-labels for concept drift adaptation. By incorporating contrastive learning techniques, we investigate whether the model's ability to select informative and representative pseudo-labeled samples is enhanced. 

\item RQ2) \textit{To what extent can pseudo-label-based adaptation reduce the frequency of annotations required in active learning?}

We analyze the potential reduction in annotation frequency achieved through pseudo-label-based concept drift adaptation in the active learning process. By comparing the performance of our adaptation algorithm with traditional active learning approaches that solely rely on annotated ground truth labels, we identify the reduction in annotation requirements. 

\item RQ3) \textit{How do pseudo labels with neural networks perform compared to prior attempts at automated concept drift adaptation?}

We compare the proposed method against the state-of-the-art concept drift adaptation algorithm for Android malware detection DroidEvolver++~\cite{kan2021investigating}.  We show that the proposed neural network-based method outperforms it significantly.

\end{enumerate}

To assess the effectiveness of our approach, we conduct experiments using two malware detection datasets—one focusing on Android~\cite{chen2023continuous} and the other on Windows platforms~\cite{2018arXiv180404637A}. By reporting and analyzing our experimental findings, we contribute insights into the efficacy of using pseudo-labels in conjunction with active learning for concept drift adaptation in malware detection.
